A Distributed MAC Protocol for Cooperation in Random Access Networks

WLAN is one of the most successful applications of wireless communications in daily life because of low cost and ease of deployment. The enabling technique for this success is the use of random access schemes for the wireless channel. Random access requires minimal coordination between the nodes, which considerably reduces the cost of the infrastructure. Recently, cooperative communication in wireless networks has been of increasing interest because it promises higher rates and reliability. An additional MAC overhead is necessary to coordinate the nodes to allow cooperation and this overhead can possibly cancel out the cooperative benefits. In this work, a completely distributed protocol is proposed that allows nodes in the network to cooperate via Two-Hop and Decode-and-Forward for transmitting their data to a common gateway node. It is shown that high throughput gains are obtained in terms of the individual throughput that can be guaranteed to any node in the network. These results are validated by Monte Carlo simulations.

==> Makefile <==
PROJECT=min-rate
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps

default: $(PROJECT).tex

clean:
	rm -f $(TMPFILES);
clean_pdf:
	rm -f $(PROJECT).pdf;

$(PROJECT).tex: clean_pdf
	pdflatex $(PROJECT);

$(PROJECT).texAll: clean
	ps4pdf $(PROJECT);
	pdflatex $(PROJECT);
	bibtex $(PROJECT);
	pdflatex $(PROJECT);
	pdflatex $(PROJECT);
	pdflatex $(PROJECT);

bib:	
	bibtex $(PROJECT);

literatur:
	cp ../references/Literatur.bib ./;
	cp ../references/confs-jrnls.bib ./;

final: clean clean_pdf
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	bibtex $(PROJECT);
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $(PROJECT).ps;
	pdffonts $(PROJECT).pdf;

arxiv:
	rm -f $(PROJECT).aux $(PROJECT).blg $(PROJECT).dvi $(PROJECT).log $(PROJECT).pdf $(PROJECT).ps *.bib *~ .*.xml;



==> acknowledgment.tex <==
\section*{Acknowledgment}
This work was partly supported by the UMIC excellence cluster of RWTH
Aachen University.
